Proof of the Kakeya set conjecture over rings of integers modulo square-free $N$

A Kakeya set $S \subset (\mathbb{Z}/N\mathbb{Z})^n$ is a set containing a line in each direction. We show that, when $N$ is any square-free integer, the size of the smallest Kakeya set in $(\mathbb{Z}/N\mathbb{Z})^n$ is at least $C_{n,\epsilon} N^{n - \epsilon}$ for any $\epsilon$ -- resolving a special case of a conjecture of Hickman and Wright. Previously, such bounds were only known for the case of prime $N$. We also show that the case of general $N$ can be reduced to lower bounding the $\mathbb{F}_p$ rank of the incidence matrix of points and hyperplanes over $(\mathbb{Z}/p^k\mathbb{Z})^n$.

==> abstract.tex <==
\begin{abstract}
Blah blah blah
\end{abstract}

==> earlierWork.tex <==
\section{Previous Work}
The problem of lower bounding sizes of Kakeya sets for rings $\Z/N\Z$ for squarefree $N$ is discussed in \cite{dvir2010incidence}. The regular polynomial method argument involves lower bounding the size of Kakeya sets with the dimension of the space of polynomials of some fixed degree. This method fails in this setting because the Chinese Remainder Theorem leads to the decomposition of polynomials over $\Z/N\Z$. This leads to the space of polynomials being too small to give us good bounds. Our arguments here circumvent this problem. 

The problem of lower bounding Kakeya sets sizes for rings $\Z/p^k\Z$ and $\F_q[x]/\langle x^k\rangle$ was first proposed in \cite{ellenberg2010kakeya}. They suggested these problems as the next model problem towards understanding the Euclidean case of the Kakeya conjecture. A lower bound of $p^{2k}k^{-1}$ for Kakeya sets in $(\Z/p^k\Z)^2$ was proven in \cite{dummit_hablicsek_2013}. In \cite{hickman2018fourier} they study the case of the $p$-adic integers $\Z_p$. Bounds over the $p$-adics imply bounds over $\Z/p^k\Z$ for all $k$ and vice-versa. They look at a stronger version of the Kakeya problem involving maximal operators and use tools applied in the Euclidean case to find bounds over the $p$-adics which in turn gives them bounds over $\Z/p^k\Z$. In particular, they can get a bound of the order of $p^{kn/2}$ for Kakeya sets in $(\Z/p^k\Z)^n$.

\Mnote{I think the arithmetic Kakeya stuff would be an alternate route to get bounds in this setting. Do you know what papers to cite for those?}

==> prelimnary.tex <==
\section{Preliminaries}
% \subsection{Some known facts about finite fields and tensor products}
For a natural number $r$, let $[r]=\{1,\hdots, r\}$.

Let $q$ be a prime power and $\F_q$ represent the finite field of size $q$. We let $\F_q[x_1,\hdots,x_n]_{=d}$ represent the vector space of homogenous $n$-variate degree $d$ polynomials over $\F_q$ and $\F_q[x_1,\hdots,x_n]_{\le d}$ refer to the space of degree at most $d$ polynomials. We let $\delta_{n,d}=\binom{n+d-1}{n-1}$ which is the dimension of the space $ \F_q[x_1,\hdots,x_n]_{=d}$ and $\Delta_{n,d}=\binom{n+d}{n}$ which is the dimension of the space $\F_q[x_1,\hdots,x_n]_{\le d}$. 

Given a finite ring $R$, a field $\F$, and a natural number $n$, we define $\F^{|R^n|}$ as a $|R|^n$ dimensional vector space over $\F$ whose elements are represented by column vectors of size $|R|^n$ indexed by points in $R^n$. We can similarly define $\Z^{|R^n|}$. 

We also define $\left(\F^{|R^n|}\right)^T$ (similarly $\left(\Z^{|R^n|}\right)^{T}$) as the space of the transpose of all elements in $\F^{|R^n|}$. $\left(\F^{|R^n|}\right)^T$ is then the space of all row vectors with size $|R^n|$ indexed by points in $R^n$.

Now given a subset $A\subseteq R^n$, we let $\Ind_A\in \left(\F^{|R^n|}\right)^T$ refer to the indicator vector of $A$ over $R^n$ where the entry corresponding to the entry $x\in R^n$ is $1$ if $x\in A$ and $0$ otherwise. Multiplying $\Ind_A$ with column vectors in $\F^{|R^n|}$ gives us a linear map $\Ind_A\cdot:\F^{|R^n|}\rightarrow \F$ where $\F$ can be any field. As before $\F$ can be replaced by $\Z$ too. In general we use $A\cdot B$ to refer to the product of two matrices $A$ and $B$.

For an element $b\in R^n$ we define the sets $H_b=\{x|\langle x,b\rangle =0\}\subseteq R^n$ and $\overline{H}_b=\{x|\langle x,b\rangle \ne 0\}\subseteq R^n$. We note non-zero vectors $b$ which are unit multiples of each other will define the same sets $H_b,\overline{H}_b$.


% This means $\Ind_A$ acts as a linear function over the space $\Z^{|R^n|}$. We can also lift $\Ind_A$ to any field $\F$ to get a function $\Ind_A\otimes \F: \F^{|R^n|}\rightarrow \F$. We will hide the $\otimes \F$ notation whenever the field we are working over is clear from context.

We will use a simple corollary of the following result from~\cite{goethalsDel1968,macwilliams1968p,smith1969p}.

\begin{thm}[$p$-rank of the vector space generated by indicator functions of hyperplanes]\label{thm:pRankSubs}
Given a natural number $n$ and a prime power $q=p^t$ where $p$ is a prime and $t$ is a natural number, the $\F_p$-vector space generated by the indicator vectors $\Ind_{H_b}\in \left(\F_p^{|\F_q^n|}\right)^T$ for all $b\in \P \F_q^n$ has dimension $$\Delta_{n,p-1}^t+1=\binom{p+n-1}{n}^t+1.$$
\end{thm}

\begin{cor}\label{cor:pRankSubs}
Given a natural number $n$ and a prime power $q=p^t$ where $p$ is a prime and $t$ is a natural number, the $\F_p$-vector space generated by the indicator vectors $\Ind_{\overline{H}_b}\in \left(\F_p^{|\F_q^n|}\right)^T$ for all $b\in \P\F_q^n$ has dimension at least $$\Delta_{n,p-1}^t=\binom{p+n-1}{n}^t.$$
\end{cor}
\begin{proof}
Consider a matrix $M$ whose rows are indexed by elements in $b\in \F_{q}^n$ and the row indexed by $b$ is the indicator vector $\Ind_{\overline{H}_b}$. Let $A$ be the all ones matrix with the same size as $M$. $A-M$ is then a matrix whose rows are indexed by elements $b \in \F_p^n$ and the row corresponding to $b$ is the indicator function of the set $H_b$. Theorem \ref{thm:pRankSubs} and the fact that $A$ is rank one then gives the required dimension lower bound. 
\end{proof}



We will also use the well known Chinese remainder theorem.

\begin{thm}[Chinese Remainder Theorem]\label{thm:Chinese}
For distinct primes $p_1,\hdots,p_r$ and $N=p_1\hdots p_r$, we have the isomorphism
$$\Z/N\Z\cong \bigoplus\limits_{t=1}^r \F_{p_t},$$
where the isomorphism takes a number $x$ in $\Z/N\Z$ and maps it to the tuple $(x \text{ }(\text{mod }p_t))_{t=1}^r$.
\end{thm}

We will use this theorem for rings $\Z/N\Z$ where $N=p_1 p_2 \hdots p_r$ for distinct primes $p_1,p_2,\hdots,p_r$. We get a number of equivalences between geometric objects of $(\Z/N\Z)^n$ and \\ $\F_{p_1}^n\times \hdots \times \F_{p_r}^n$ directly from Theorem \ref{thm:Chinese}.

\begin{cor}[Geometric dictionary between $(\Z/p_1\hdots p_r\Z)^n$ and $\F_{p_1}^n\times \hdots \times \F_{p_r}^n$]\label{cor:geometricDictionary}
Given distinct primes $p_1,p_2,\hdots,p_r$, a natural number $n$, $N=p_1 \hdots p_r$ and the ring $R=\Z/N\Z$, we have the following equivalences between the spaces $R^n$ and $\F_{p_1}^n\times \hdots\times  \F_{p_r}^n$,
\begin{enumerate}
    \item Every point $x \in R^n$ is represented by a tuple of points $(x_1,x_2,\hdots,x_r)\in \F_{p_1}^n\times \F_{p_2}^n \hdots \times \F_{p_r}^n$ via the map $x\rightarrow (x \text{ }(\text{mod }p_t))_{t=1}^r$.
    \item The set $\P R^n$ is isomorphic to $\P \F_{p_1}^n\times\hdots\times \P\F_{p_r}^n$ via the map $b\rightarrow (b \text{ }(\text{mod }p_t))_{t=1}^r$.
    \item Every line $L \subseteq R^n$ with direction $b\in \P R^n$ is represented by a product of lines $L_1\times L_2 \times \hdots\times L_r \subseteq \F_{p_1}^n\times \F_{p_2}^n\hdots \times \F_{p_r}^n$ where $L_i$ is a line in $\F_{p_i}^n$ with direction $b_i\in \P \F_{p_i}^n$ for $i\in [r]$. $L_i$ is obtained from $L$ via the map $x\rightarrow (x \text{ }(\text{mod }p_i))$. 
    \item The indicator vector of a line $L\subseteq R^n$, $\Ind_L\in \left(\Z^{|R^n|}\right)^T$ equals the tensor product of the indicator vectors $\Ind_{L_1}\otimes \hdots \otimes \Ind_{L_r}\in \left(\Z^{|\F_{p_1}^n|}\right)^T\otimes\hdots \otimes \left(\Z^{|\F_{p_r}^n|}\right)^T=\left(\Z^{|\F_{p_1}^n\times\hdots \times \F_{p_r}^n|}\right)^T$. This result holds even if we lift the vectors to some field $\F$.
\end{enumerate}
\end{cor}
% : \Z^{|\F_{p_1}^n|}\times\hdots \Z^{|\F_{p_r}^n|}=\Z^{|\F_{p_1}^n\times\hdots \times \F_{p_r}^n|} \rightarrow \Z
We list some facts about tensor products.

\begin{fact}[The tensor product of two basis]\label{fact:TensorBasis}
Given a basis $\{v_1,v_2,\hdots,v_n\}$ for a vector space $V$ and a basis $\{u_1,\hdots, u_m\}$ for a vector space $U$, we have that $\{v_i\otimes u_j\}_{i\in [n],j\in [m]}$ is a basis for $V\otimes U$.
\end{fact}

\begin{fact}[The tensor product of two maps]\label{fact:tensorMaps}
Given vector spaces $V_1,V_2,U_1,U_2$, linear maps $A: V_1\rightarrow U_1$ and $B:V_2\rightarrow U_2$, we have the map $A\otimes B: V_1\otimes V_2\rightarrow U_1\otimes U_2$ which acts on elements $x\otimes y \in V_1\otimes V_2$ to output $A(x)\otimes B(y)$. Also given matrix representations of $A$ and $B$ in some basis, $A\otimes B$ can be written as the tensor (Kronecker) product of the two matrices in the tensored basis. Finally, given maps $C:U_1\rightarrow W_1$ and $D:U_2\rightarrow W_2$ for vector spaces $W_1,W_2$, we have $(C\otimes D)\cdot (A\otimes B)=(C\cdot A)\otimes (D\cdot B)$.
\end{fact}

We will now prove a simple lemma we need.

\begin{lem}[Rank lower bounds for product like spaces]\label{lem:tensorProductSpaceBound}
Given finite dimensional vector spaces $V$ and $U$ over a field $\F$, let $A=\{v_1,v_2,\hdots,v_n\}\subseteq V$ be a set of linearly independent vectors and $B_1,B_2,\hdots,B_n \subseteq U$ each of which spans a subspace of dimension at least $k$, then the space spanned by the vectors $\bigcup_{i=1}^n\{v_i\otimes y| y\in B_i\}$ has dimension at least $nk$ in $V\otimes U$
\end{lem}
\begin{proof}
Let $C=\{c_1,\hdots,c_m\}$ be some basis of $U$ where we let $m$ be the dimension of $U$. Fact \ref{fact:TensorBasis} shows that $v_i\otimes c_j$ where $i\in [n]$ and $j\in [m]$ form a linearly independent set of vectors in $V\otimes U$. For each set $B_i$ we can find a set of $k$ linearly independent vectors $B'_i=\{b^i_1,\hdots,b^i_k\}$ all of which can be written as a linear combination of elements in $C$.

We will show the set of vectors $\bigcup_{i=1}^n\{v_i\otimes y| y\in B'_i\}$ is linearly independent to prove the lemma. Let us consider a linear combination of these vectors which equals $0$,
$$\sum_{i=1}^n \sum_{j=1}^k \alpha_{i,j} v_i\otimes b^i_j=0,$$
where $\alpha_{i,j}$ are scalars. This means,
\begin{align}
\sum\limits_{i=1}^n v_i\otimes (\sum_{j=1}^k \alpha_{i,j}  b^i_j)=0. \label{eq:tensorProductLemma}
\end{align}

Consider the linear projection operator $P_i$ defined as,
$$P_i(v_j\otimes c_k) =
\left\{
	\begin{array}{ll}
		c_k  & \mbox{if } j = i \\
		0 & \mbox{if } j \ne i
	\end{array}
\right. $$
Applying $P_i$ on \eqref{eq:tensorProductLemma} gives us,
$$ \sum_{j=1}^k \alpha_{i,j} b^i_j=0.$$
As $b^i_1,\hdots,b^i_k$ are linearly independent we have $\alpha_{i,j}=0$ for all $i$ and $j$.
\end{proof}




% With this perspective in mind we have the following simple Corollary.

% \begin{cor}[Lines along the same direction give similar $C(L,m)$ maps] Given any two lines $L_1$ and $L_2$ in $\F_p^n$ which are both parallel to the direction $b\in \F_p^n\setminus \{0\}$ and some natural number $m$ the operators $C(L_1,b,m)$ and $C(L_2,b,m)$ act identically over the subspace of evaluations of Hasse derivative of weight strictly less than $m$ of polynomials of degree strictly less than $mp$.
% \end{cor}

% We will now construct a matrix associated with a Kakeya set $S$ using a family of $C(L,k)$ maps where $L$ is contained in $S$. 

% \begin{define}[Matrix of derivatives along lines]
% Given natural numbers $k,n$, a prime $p$ and a Kakeya set $S\subseteq \F_p^n$ we define the $k$th order matrix of derivatives along lines $D_S(k)$ as the matrix obtained by concatenating along columns the set of all matrices $C(L,k)$ for all lines $L$ contained in $S$.
% \end{define}

% We now state a result about how these maps on different directions act on polynomials. This is the key argument in \cite{dvir2013extensions} in disguise.

% \begin{thm}
% Given natural numbers $k,n$, a prime $p$ and a Kakeya set $S\subseteq \F_p^n$ the map $P_S(k)$ composed with $\text{Eval}(\F^n_p,2k-k/p)$ acts injectively over $\F_p[x_1,\hdots,x_n]_{=kp-1}$.
% \end{thm}
% \begin{proof}
% Using Lemma \ref{lem:infitDerLine} we see that the image of any degree $kp-1$ homogenous polynomial under the map $\text{Eval}(\F^n_p,2k-k/p)$ and $P_S(k)$ will be the same as the image of $\text{Eval}(\F^n_p,k)$. Using Corollary \ref{cor:extMultFourier} we know that $\text{Eval}(\F^n_p,k)$ acts injectively over $\F_p[x_1,\hdots,x_n]_{=kp-1}$.
% \end{proof}

% We now prove an analogue of the lower bound in Lemma \ref{lem:rankSizeLine} for this setting.

% \begin{lem}[Rank-Size relation for $P_S(k)$]\label{lem:rankSizeProject}
% For any minimal Kakeya Set $S\subseteq \F_p^n$,
% $$|S|\binom{m+n-1}{n}\ge \text{rank}(P_S(k),\F_p),$$
% where $m=2k-k/p$.
% \end{lem}
% \begin{proof}
% The lower bounds follows from noting the number of non-zero columns in $P_S(k)$ is equal to $|S|\binom{m+n-1}{n}$ because each point in $S$ contributes $\binom{m+n-1}{n}$ many non-zero columns corresponding to the Hasse derivatives of weight strictly less than $m$ on that point.
% \end{proof}


% \begin{define}[Matrix of projections along lines]
% Given a Kakeya set $S$ and a number $m>0$ we construct the matrix of projections $P_S(m)$ of weight $m$ by concatenating matrices $C(L,m)$ for each line $L$ contained in $S$ along columns.
% \end{define}

% We now prove an analogue of the lower bound in Lemma \ref{lem:rankSizeLine} in this setting.

% \begin{lem}[Rank-Size relation for $P_S(m)$]\label{lem:rankSizeProject}
% For any minimal Kakeya Set $S\subseteq \F_p^n$,
% $$|S|\binom{m+n-1}{n}\ge \text{rank}(P_S(m),\F_p).$$
% \end{lem}
% \begin{proof}
% The lower bounds follows from noting the number of non-zero columns in $P_S(m)$ is equal to $|S|\binom{m+n-1}{n}$ because each point in $S$ contributes $\binom{m+n-1}{n}$ many non-zero columns corresponding to the Hasse derivatives of weight strictly less than $m$ on that point.
% \end{proof}



